Model Synthesis for Zero-Shot Model Attribution

Nowadays, generative models are shaping various fields such as art, design, and human-computer interaction, yet accompanied by challenges related to copyright infringement and content management. In response, existing research seeks to identify the unique fingerprints on the images they generate, which can be leveraged to attribute the generated images to their source models. Existing methods, however, are constrained to identifying models within a static set included in the classifier training, failing to adapt to newly emerged unseen models dynamically. To bridge this gap, we aim to develop a generalized model fingerprint extractor capable of zero-shot attribution, effectively attributes unseen models without exposure during training. Central to our method is a model synthesis technique, which generates numerous synthetic models mimicking the fingerprint patterns of real-world generative models. The design of the synthesis technique is motivated by observations on how the basic generative model's architecture building blocks and parameters influence fingerprint patterns, and it is validated through two designed metrics that examine synthetic models' fidelity and diversity. Our experiments demonstrate that this fingerprint extractor, trained solely on synthetic models, achieves impressive zero-shot generalization on a wide range of real-world generative models, improving model identification and verification accuracy on unseen models by over 40% and 15%, respectively, compared to existing approaches.

==> Figures/1v1_tsne.tex <==
\newcommand\tsnefigurewidth{0.25}

\begin{figure*}
\setlength{\abovecaptionskip}{2mm}
\centering
\begin{minipage}{\tsnefigurewidth\linewidth}
    \includegraphics[width=\linewidth]{PAMI/Images/1v1_tsne_0415/cnn_gan_data.pdf}
\end{minipage}
\begin{minipage}{\tsnefigurewidth\linewidth}
    \includegraphics[width=\linewidth]{PAMI/Images/1v1_tsne_0415/transformer_gan_data.pdf}
\end{minipage}
\begin{minipage}{\tsnefigurewidth\linewidth}
    \includegraphics[width=\linewidth]{PAMI/Images/1v1_tsne_0415/vae_data.pdf}
\end{minipage}
\vspace{4pt}
\begin{minipage}{\tsnefigurewidth\linewidth}
    \centering
    \figtext{(a) GAN (CNN\_based)}
\end{minipage}
\begin{minipage}{\tsnefigurewidth\linewidth}
    \centering
    \figtext{(b) GAN (Transformer\_based)}
\end{minipage}
\begin{minipage}{\tsnefigurewidth\linewidth}
    \centering
    \figtext{(c) VAE}
\end{minipage}

\begin{minipage}{\tsnefigurewidth\linewidth}
    \includegraphics[width=\linewidth]{PAMI/Images/1v1_tsne_0415/flow_data.pdf}
\end{minipage}
\begin{minipage}{\tsnefigurewidth\linewidth}
    \includegraphics[width=\linewidth]{PAMI/Images/1v1_tsne_0415/diffusion_data.pdf}
\end{minipage}
\begin{minipage}{\tsnefigurewidth\linewidth}
    \includegraphics[width=\linewidth]{PAMI/Images/1v1_tsne_0415/T2I_data.pdf}
\end{minipage}
\vspace{4pt}
\begin{minipage}{\tsnefigurewidth\linewidth}
    \centering
    \figtext{(d) Flow}
\end{minipage}
\begin{minipage}{\tsnefigurewidth\linewidth}
    \centering
    \figtext{(e) Diffusion}
\end{minipage}
\begin{minipage}{\tsnefigurewidth\linewidth}
    \centering
    \figtext{(f) Text2Image}
\end{minipage}
\caption{Feature visualization of models in Table~\ref{tab:dataset}. Although the fingerprint extractor is trained solely on synthetic models, it could extract distinct fingerprints from actual generative models including GAN, VAE, Flow, Diffusion, and state-of-the-art Text2Image models.}
\label{fig:1v1_tsne}
\end{figure*}


==> Figures/1v1_verification.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{PAMI/Images/1v1_verification.pdf}
\caption{The 1v1 model verification scenario.}
\label{fig:1v1_verification}
\end{figure}


==> Figures/1vn_result.tex <==
\begin{figure}[t]
\setlength{\abovecaptionskip}{2mm}
\centering

\begin{minipage}{0.48\linewidth}
    \includegraphics[width=\linewidth]{Images/1vn_result/acc_along_dataset_size.pdf}
\end{minipage}
\begin{minipage}{0.48\linewidth}
    \includegraphics[width=\linewidth]{Images/1vn_result/auc_along_dataset_size.pdf}
\end{minipage}
% \begin{minipage}{0.25\linewidth}
%     \includegraphics[width=\linewidth]{Images/1v1_tsne_v2/sd_1and2_version2.pdf}
% \end{minipage}

\begin{minipage}{0.48\linewidth}
    \centering
    \figtext{(a)}
\end{minipage}
\begin{minipage}{0.48\linewidth}
    \centering
    \figtext{(b)}
\end{minipage}
% \begin{minipage}{0.25\linewidth}
%     \centering
%     \figtext{(c)}
% \end{minipage}
\caption{(a)(b) Open-set model identification accuracy and closed/open discrimination AUC along with dataset sizes.}
\label{fig:1vn_result}
\end{figure}

 % (c) Feature space visualization for different versions of stable diffusion models.

==> Figures/base1.tex <==

\begin{figure}[h]
\setlength{\abovecaptionskip}{2mm}
\centering

\begin{minipage}{0.48\linewidth}
    \centering
    \figtext{Seen Models}
\end{minipage}
\begin{minipage}{0.48\linewidth}
    \centering
    \figtext{Unseen Models}
\end{minipage}

\begin{minipage}{0.48\linewidth}
\includegraphics[width=\linewidth]{Images/1v1_tsne_0415/attnet_4000_test.pdf}
\end{minipage}
\begin{minipage}{0.48\linewidth}
\includegraphics[width=\linewidth]{Images/1v1_tsne_0415/attnet_4000_test_out.pdf}
\end{minipage}

\caption{Feature visualization results by Yu et al.~\cite{yu2019attributing}} 
\label{fig:base1}
\end{figure}


==> Figures/base2.tex <==

\begin{figure}[h]
\setlength{\abovecaptionskip}{2mm}
\centering

\begin{minipage}{0.48\linewidth}
    \centering
    \figtext{Seen Models}
\end{minipage}
\begin{minipage}{0.48\linewidth}
    \centering
    \figtext{Unseen Models}
\end{minipage}

\begin{minipage}{0.48\linewidth}
\includegraphics[width=\linewidth]{Images/1v1_tsne_0415/dna_4000_test.pdf}
\end{minipage}
\begin{minipage}{0.48\linewidth}
\includegraphics[width=\linewidth]{Images/1v1_tsne_0415/dna_4000_test_out.pdf}
\end{minipage}

\caption{Feature visualization results by DNA-Det~\cite{yang2022aaai}} 
\label{fig:base2}
\end{figure}


==> Figures/base3.tex <==

\begin{figure}[h]
\setlength{\abovecaptionskip}{2mm}
\centering

\begin{minipage}{0.48\linewidth}
    \centering
    \figtext{Seen Models}
\end{minipage}
\begin{minipage}{0.48\linewidth}
    \centering
    \figtext{Unseen Models}
\end{minipage}

\begin{minipage}{0.48\linewidth}
\includegraphics[width=\linewidth]{Images/1v1_tsne_0415/repmix_4000_test.pdf}
\end{minipage}
\begin{minipage}{0.48\linewidth}
\includegraphics[width=\linewidth]{Images/1v1_tsne_0415/repmix_4000_test_out.pdf}
\end{minipage}

\caption{Feature visualization results by RepMix~\cite{bui2022repmix}} 
\label{fig:base3}
\end{figure}


==> Figures/block_exchange.tex <==


\begin{figure}[t]
\centering

% \begin{minipage}{0.12\linewidth}
%     \centering
%     \figtext{\quad}
% \end{minipage}
\begin{minipage}{0.24\linewidth}
    \centering
    \figtext{Testing I}
\end{minipage}
\begin{minipage}{0.24\linewidth}
    \centering
    \figtext{Exchange \\the Last One}
\end{minipage}
\begin{minipage}{0.24\linewidth}
    \centering
    \figtext{Exchange \\the Last Two}
\end{minipage}
\begin{minipage}{0.24\linewidth}
    \centering
    \figtext{Exchange \\the Last Three}
\end{minipage}


% \begin{minipage}{0.12\linewidth}
%     \centering
%     \figtext{Nearest}
% \end{minipage}
\begin{minipage}{1\linewidth}
\includegraphics[width=\linewidth]{PAMI/Images/cm_progan_nearest.png}
\end{minipage}
% \begin{minipage}{0.12\linewidth}
%     \centering
%     \figtext{Bilinear}
% \end{minipage}
\begin{minipage}{1\linewidth}
\includegraphics[width=\linewidth]{PAMI/Images/cm_progan_bilinear.png}
\end{minipage}


\caption{Spectral effects of exchanging generative blocks.} 
\label{fig:block_exchange}
\end{figure}


==> Figures/conv.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{PAMI/Images/conv.pdf}
    \caption{Frequency illustration on how convolution leaves fingerprints.}
    \label{fig:conv}
\end{figure}

==> Figures/fingerprint_decay.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{PAMI/Images/fingerprint_decay.pdf}
    \caption{The fingerprint decay phenomenon between generative blocks within a StyleGAN2 face generator.}
    \label{fig:fingerprint_decay}
\end{figure}

==> Figures/generalization.tex <==

\begin{figure*}
\centering
% \begin{minipage}{0.1\linewidth}
%     \centering
%     \figtext{\quad}
% \end{minipage}

\begin{minipage}{0.48\linewidth}
    \centering
    \figtext{Classical Models}
\end{minipage}
\begin{minipage}{0.48\linewidth}
    \centering
    \figtext{Emerging Models}
\end{minipage}

% \vspace{4pt}
% \begin{minipage}{0.1\linewidth}
%     \centering
%     \figtext{\textbf{POSE}}
% \end{minipage}
\begin{minipage}{0.24\linewidth}
    \includegraphics[width=\linewidth]{Images/1v1_tsne_0415/pose_4000_test.pdf}
\end{minipage}
\begin{minipage}{0.24\linewidth}
    \includegraphics[width=\linewidth]{Images/1v1_tsne_0415/syn_4000_test.pdf}
\end{minipage}
\begin{minipage}{0.24\linewidth}
    \includegraphics[width=\linewidth]{Images/1v1_tsne_0415/pose_4000_test_out.pdf}
\end{minipage}
\begin{minipage}{0.24\linewidth}
    \includegraphics[width=\linewidth]{Images/1v1_tsne_0415/syn_4000_test_out.pdf}
\end{minipage}

\begin{minipage}{0.98\linewidth}
    \includegraphics[width=\linewidth]{Images/legend.pdf}
\end{minipage}

\begin{minipage}{0.24\linewidth}
    \centering
    \figtext{(a) POSE}
\end{minipage}
\begin{minipage}{0.24\linewidth}
    \centering
    \figtext{(b) Ours (Only-Syn)}
\end{minipage}
\begin{minipage}{0.24\linewidth}
    \centering
    \figtext{(c) POSE}
\end{minipage}
\begin{minipage}{0.24\linewidth}
    \centering
    \figtext{(d) Ours (Only-Syn)}
\end{minipage}
% \begin{minipage}{0.3\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{Images/1v1_tsne_0415/legend_unseen.pdf}
% \end{minipage}

% \begin{minipage}{0.48\linewidth}
%     \centering
%     \figtext{(a) Conventional method}
% \end{minipage}
% \begin{minipage}{0.48\linewidth}
%     \centering
%     \figtext{(b) Our method}
% \end{minipage}
\caption{Compare existing method POSE~\cite{yang2023progressive} and our method in attributing classical and emerging models. POSE is trained on samples from classical models. As depicted in the figure, it effectively extracts distinct fingerprint patterns from these seen models (a), while struggles to generalize this capability to unseen, emerging models (c). In contrast, our method, despite not being trained on any of these testing models, demonstrates robust generalization abilities on the two groups of models (b,d).}

\label{fig:generalization}
\end{figure*}


==> Figures/generalized_attribution.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{PAMI/Images/generalized_attribution.pdf}
    \caption{Model attribution accuracy on known models and novel models in the generalized model attribution scenario varying the number of known models in training.}
    \label{fig:generalized_attribution}
\end{figure}

==> Figures/hist_tsne_compare.tex <==
% \newcommand\subfigurewidth{0.22}

% \begin{figure*}
% \setlength{\abovecaptionskip}{2mm}
% \centering
% \begin{minipage}{0.1\linewidth}
%     \centering
%     \figtext{\quad}
% \end{minipage}
% \begin{minipage}{\subfigurewidth\linewidth}
%     \centering
%     \figtext{Known Models}
% \end{minipage}
% \begin{minipage}{\subfigurewidth\linewidth}
%     \centering
%     \figtext{Novel Models}
% \end{minipage}
% \begin{minipage}{\subfigurewidth\linewidth}
%     \centering
%     \figtext{Known Models}
% \end{minipage}
% \begin{minipage}{\subfigurewidth\linewidth}
%     \centering
%     \figtext{Novel Models}
% \end{minipage}
% % \vspace{4pt}

% % \begin{minipage}{0.1\linewidth}
% %     \centering
% %     \figtext{\textbf{POSE}}
% % \end{minipage}
% % \begin{minipage}{\subfigurewidth\linewidth}
% %     \includegraphics[width=\linewidth]{PAMI/Images/1v1_tsne_0415/pose_4000_test.pdf}
% % \end{minipage}
% % \begin{minipage}{\subfigurewidth\linewidth}
% %     \includegraphics[width=\linewidth]{PAMI/Images/1v1_tsne_0415/pose_4000_test_out.pdf}
% % \end{minipage}
% \begin{minipage}{\subfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{PAMI/Images/plot_hist_0415/pose_4000_test.pdf}
% \end{minipage}
% \begin{minipage}{\subfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{PAMI/Images/plot_hist_0415/pose_4000_test_out.pdf}
% \end{minipage}
% % \vspace{4pt}

% % \begin{minipage}{0.1\linewidth}
% %     \centering
% %     \figtext{\textbf{Ours \\(Only Syn)}}
% % \end{minipage}
% % \begin{minipage}{\subfigurewidth\linewidth}
% %     \includegraphics[width=\linewidth]{PAMI/Images/1v1_tsne_0415/syn_4000_test.pdf}
% % \end{minipage}
% % \begin{minipage}{\subfigurewidth\linewidth}
% %     \includegraphics[width=\linewidth]{PAMI/Images/1v1_tsne_0415/syn_4000_test_out.pdf}
% % \end{minipage}
% \begin{minipage}{\subfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{PAMI/Images/plot_hist_0415/syn_4000_test.pdf}
% \end{minipage}
% \begin{minipage}{\subfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{PAMI/Images/plot_hist_0415/syn_4000_test_out.pdf}
% \end{minipage}
% \vspace{4pt}

% % \begin{minipage}{0.1\linewidth}
% %     \centering
% %     \figtext{\textbf{Ours\\(Fine-tune)}}
% % \end{minipage}
% % \begin{minipage}{\subfigurewidth\linewidth}
% %     \includegraphics[width=\linewidth]{PAMI/Images/1v1_tsne_0415/ft_4000_test.pdf}
% % \end{minipage}
% % \begin{minipage}{\subfigurewidth\linewidth}
% %     \includegraphics[width=\linewidth]{PAMI/Images/1v1_tsne_0415/ft_4000_test_out.pdf}
% % \end{minipage}
% % \begin{minipage}{\subfigurewidth\linewidth}
% %     \includegraphics[width=\linewidth]{PAMI/Images/plot_hist_0415/ft_4000_test.pdf}
% % \end{minipage}
% % \begin{minipage}{\subfigurewidth\linewidth}
% %     \includegraphics[width=\linewidth]{PAMI/Images/plot_hist_0415/ft_4000_test_out.pdf}
% % \end{minipage}
% % \vspace{4pt}

% \caption{Feature visualization of models in Table~\ref{tab:dataset}. Although the fingerprint extractor is trained solely on synthetic models, it could extract distinct fingerprints from actual generative models including GAN, VAE, Flow, Diffusion, and state-of-the-art Text2Image models.}
% \label{fig:hist_tsne_compare}
% \end{figure*}




\newcommand\subfigurewidth{0.43}

\begin{figure}
\centering
% \begin{minipage}{0.1\linewidth}
%     \centering
%     \figtext{\quad}
% \end{minipage}
% \begin{minipage}{\subfigurewidth\linewidth}
%     \centering
%     \figtext{Known Models}
% \end{minipage}
% \begin{minipage}{\subfigurewidth\linewidth}
%     \centering
%     \figtext{Novel Models}
% \end{minipage}
% \begin{minipage}{\subfigurewidth\linewidth}
%     \centering
%     \figtext{Known Models}
% \end{minipage}
% \begin{minipage}{\subfigurewidth\linewidth}
%     \centering
%     \figtext{Novel Models}
% \end{minipage}
% % \vspace{4pt}

\begin{minipage}{0.1\linewidth}
    \centering
    \figtext{\quad}
\end{minipage}
\begin{minipage}{\subfigurewidth\linewidth}
    \centering
    \figtext{Seen Models}
\end{minipage}
\begin{minipage}{\subfigurewidth\linewidth}
    \centering
    \figtext{Unseen Models}
\end{minipage}

\begin{minipage}{0.1\linewidth}
    \centering
    \figtext{(a)}
\end{minipage}
\begin{minipage}{\subfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{Images/plot_hist_0415/pose_4000_test.pdf}
\end{minipage}
\begin{minipage}{\subfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{Images/plot_hist_0415/pose_4000_test_out.pdf}
\end{minipage}

% \begin{minipage}{\subfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{PAMI/Images/plot_hist_0415/syn_4000_test.pdf}
% \end{minipage}
% \begin{minipage}{\subfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{PAMI/Images/plot_hist_0415/syn_4000_test_out.pdf}
% \end{minipage}

\begin{minipage}{0.1\linewidth}
    \centering
    \figtext{(b)}
\end{minipage}
\begin{minipage}{\subfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{Images/plot_hist_0415/ft_4000_test.pdf}
\end{minipage}
\begin{minipage}{\subfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{Images/plot_hist_0415/ft_4000_test_out.pdf}
\end{minipage}

\caption{Histogram of fingerprint similarity between pairs of images. In the figure, "same" refers to pairs of images generated by the same model, while "different" indicates that the images come from different generative models. We evaluate the fingerprint embeddings extracted using POSE in (a) and Ours (Fine-tune) in (b) on models that are seen and unseen.}
\label{fig:hist_tsne_compare}
\end{figure}


==> Figures/problem_setup.tex <==
\begin{figure*}
\setlength{\abovecaptionskip}{0mm}
\centering
\includegraphics[width=\linewidth]{Images/problem_setup.pdf} 
\vspace{4pt}
\begin{minipage}{0.48\linewidth}
    \centering
    \figtext{(a) Model verification}
\end{minipage}
\begin{minipage}{0.48\linewidth}
    \centering
    \figtext{(b) Open-set model identification}
\end{minipage}
\caption{Two scenarios for model attribution.}
\label{fig:problem_setup}
\end{figure*}


==> Figures/relative_volume.tex <==
\begin{figure}
    \centering    
    \includegraphics[width=0.66\linewidth]{Images/relative_volume.pdf}
    \caption{Compare the relative proportions of volume against the total volume of all synthesized models when reducing each synthesis option.}
    \label{fig:relative_volume}
\end{figure}

==> Figures/sd_transformer_tsne.tex <==

\begin{figure}[t]
\setlength{\abovecaptionskip}{2mm}
\centering

\begin{minipage}{0.5\linewidth}
% \includegraphics[width=\linewidth]{Images/1v1_tsne/7transformer.pdf}
\includegraphics[width=\linewidth]{Images/1v1_tsne/sd_similarity.png}
\end{minipage}
\begin{minipage}{0.4\linewidth}
\includegraphics[width=\linewidth]{PAMI/Images/1v1_tsne_0415/SD_data.pdf}
\end{minipage}

\begin{minipage}{0.48\linewidth}
    \centering
    \figtext{(a)}
\end{minipage}
\begin{minipage}{0.48\linewidth}
    \centering
    \figtext{(b)}
\end{minipage}

\caption{(a) Fingerprint similarity comparison. (b) Fingerprint visualization for images generated by different versions of stable diffusion models} 
\label{fig:sd_transformer_tsne}
\end{figure}


==> Figures/simulate_data.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Images/data_simulation.pdf}
\begin{minipage}{0.48\linewidth}
    \centering
    \figtext{(a)}
\end{minipage}
\begin{minipage}{0.48\linewidth}
    \centering
    \figtext{(b)}
\end{minipage}
\caption{(a) Frequency distribution pattern simulation. (b) Grid pattern simulation}
\label{fig:simulate_data}
\end{figure}


==> Figures/swap_cm.tex <==
\begin{figure}
\centering
\begin{minipage}{1\linewidth}
\includegraphics[width=\linewidth]{Images/swap_cm.pdf}
\end{minipage}
\caption{Spectral effects of swapping generative blocks.} 
\label{fig:swap_cm}
\end{figure}


==> Figures/vary_sd_configs.tex <==
\begin{figure*}
\centering
\begin{minipage}{\linewidth}
\includegraphics[width=\linewidth]{Images/robustness2.pdf}
\end{minipage}
\begin{minipage}{0.48\linewidth}
    \centering
    \figtext{(a)}
\end{minipage}
\begin{minipage}{0.48\linewidth}
    \centering
    \figtext{(b)}
\end{minipage}
\caption{(a) t-SNE visualization of extracted fingerprints from diffusion images with fixed and varied generation configurations. (b) Model identification accuracy under JPEG compression and crop resizing.} 
\label{fig:vary_sd_configs}
\end{figure*}


==> Tables/ablation_input.tex <==
\begin{table}[t!]
\centering
\caption{Ablation study on the input image for fingerprint extraction.}
\label{tab:ablation_input}
\scalebox{1.1}{
\begin{tabular}{lccccccccc}
\toprule[1pt]
\multirow{2}{*}{Input Image} & \multicolumn{2}{c}{Verification} &&\multicolumn{2}{c}{Identification} \\  
\cmidrule{2-3} \cmidrule{5-6} 
& Acc & AUC && Acc & F1 \\
\midrule
RGB & 79.22	& 87.42	& & 60.33	& 59.71 \\
Spectrum  & 83.09	& 90.76 & & 73.94& 	74.44\\
\rowcolor{gray!20} Noise Spectrum  & 89.73	& 95.69 & & 94.03& 	93.84\\
\bottomrule[1pt]
\end{tabular}}
\end{table}



==> Tables/ablation_loss.tex <==
\begin{table}[htbp]
\centering
\caption{Ablation study on loss function.}
\label{tab:ablation_loss}
\scalebox{1.2}{
\begin{tabular}{lccccccccc}
\toprule[1pt]
\multirow{2}{*}{Loss} & \multicolumn{2}{c}{Verification} &&\multicolumn{2}{c}{Identification} \\  
\cmidrule{2-3} \cmidrule{5-6} 
& Acc & AUC && Acc & F1 \\
\midrule
CE &   & \\
Triplet  &  \\
CE+Triplet  & \\
\bottomrule[1pt]
\end{tabular}}
\end{table}



==> Tables/result_1v1_verification.tex <==
\begin{table*}[t!]
% \setlength\tabcolsep{4pt}
\centering
\caption{Model verification performance under different sample number. The model verification accuracies reach over 95\% with only 10 samples.}
\label{tab:result_1v1_verification}
\begin{tabular}{lccccccccccccccccccccc}
\toprule[1pt]
\multirow{2}{*}{$N_{S}$}  &  \multirow{2}{*}{Method} & \multicolumn{2}{c}{GAN} & & \multicolumn{2}{c}{VAE}  & & \multicolumn{2}{c}{Flow} & & \multicolumn{2}{c}{Diffusion} & & \multicolumn{2}{c}{Text2Image} & & \multicolumn{2}{c}{All}\\  
\cmidrule{3-4} \cmidrule{6-7} \cmidrule{9-10}  \cmidrule{12-13} \cmidrule{15-16} \cmidrule{18-19} 
& & Acc  & AUC  & &  Acc  & AUC & & Acc  & AUC  & &  Acc & AUC  & & Acc  & AUC & & Acc  & AUC  \\
\midrule
\multirow{2}{*}{1} & PRNU~\cite{marra2019gans} &  62.03	& 65.02	& & \textbf{82.39}	& \textbf{88.66}	& & 61.23	& 65.09	& & 51.29	& 51.28	& & 56.05	& 56.87	& & 64.52	& 67.76 \\
& Ours & 
\textbf{81.06}	&\textbf{89.04}	&&72.64&	79.47	&&\textbf{99.86}&	\textbf{100.00}	&&\textbf{74.03}&	\textbf{81.90}	&&\textbf{77.14}	&\textbf{85.57}	&&\textbf{83.49}&	\textbf{91.06}\\
\midrule
\multirow{2}{*}{5} & PRNU~\cite{marra2019gans}& 79.25	& 84.95	& & \textbf{99.60}	& \textbf{99.97}	& & 76.18	& 80.48	& & 55.8	& 57.5	& & 62.74& 	65.53	& & 69.93	& 74.34 \\
& Ours & \textbf{95.24}	&\textbf{98.61}	&& 93.72	& 98.62	&&\textbf{100.00}	&\textbf{100.00}&&	\textbf{92.87}	&\textbf{98.10} &&\textbf{96.07}&	\textbf{99.31}	&&\textbf{96.22}&	\textbf{99.12} \\
\midrule
\multirow{2}{*}{10} & PRNU~\cite{marra2019gans}  & 84.63	& 89.91& & 	\textbf{100.00}	& \textbf{100.00}	& & 79.25	& 85.84& & 	59.71	& 62.57	& & 70.20 & 	73.94& & 	73.20	& 78.31 \\
& Ours & \textbf{97.21}	&\textbf{99.46}	&&98.47	&99.91	&&\textbf{100.00}	&\textbf{100.00}	&& \textbf{97.71}	&\textbf{99.76}	&&\textbf{98.73}&	\textbf{99.93}&&	\textbf{98.24}	&\textbf{99.75} \\
\bottomrule[1pt]
\end{tabular}
\end{table*}



==> Tables/result_1v1_verification2.tex <==
% \begin{table}[htbp]
% \setlength\tabcolsep{4pt}
% \centering
% \caption{Model verification performance under different sample number. The model verification accuracies reach over 95\% with only 10 samples.}
% \label{tab:result_1v1_verification2}
% \scalebox{0.8}{
% \begin{tabular}{lccccccccccccccccccccc}
% \toprule[1pt]
% \multirow{2}{*}{$N_{S}$}  &  \multirow{2}{*}{Method} & \multicolumn{2}{c}{Known models} & & \multicolumn{2}{c}{Unknown models}  & & \multicolumn{2}{c}{All models} \\ 
% \cmidrule{3-4} \cmidrule{6-7} \cmidrule{9-10}  
% & & Acc  & AUC  & &  Acc  & AUC & & Acc  & AUC \\
% \midrule
% \multirow{6}{*}{1} & Yu et al.~\cite{yu2019attributing} &  \\
% & DCT-CNN~\cite{} & \\
% & DNA-Det~\cite{} & \\
% & POSE~\cite{} & \\
% & Ours~\cite{} & \\
% & Ours w/o train & \\
% \midrule
% \multirow{6}{*}{5} & Yu et al.~\cite{yu2019attributing} &  \\
% & DCT-CNN~\cite{} & \\
% & DNA-Det~\cite{} & \\
% & POSE~\cite{} & \\
% & Ours~\cite{} & \\
% & Ours w/o train & \\
% \midrule
% \multirow{6}{*}{10} & Yu et al.~\cite{yu2019attributing} &  \\
% & DCT-CNN~\cite{} & \\
% & DNA-Det~\cite{} & \\
% & POSE~\cite{} & \\
% & Ours~\cite{} & \\
% & Ours w/o train & \\
% \bottomrule[1pt]
% \end{tabular}}
% \end{table}


\begin{table}[htbp]
\centering
\caption{Model verification performance under different sample number. The model verification accuracies reach over 95\% with only 10 samples.}
\label{tab:result_1v1_verification2}
\begin{tabular}{lccccccccccc}
\toprule[1pt]
\multirow{2}{*}{Method} & \multicolumn{2}{c}{Known models} & & \multicolumn{2}{c}{Unknown models} \\ 
\cmidrule{2-3} \cmidrule{5-6} 
& Acc  & AUC  & &  Acc  & AUC \\
\midrule
DCT-CNN~\cite{frank2020leveraging} & 66.86 & 74.21 && 67.36 & 74.23\\
Yu et al.~\cite{yu2019attributing} &  81.24 & 88.90 && 78.45 & 85.98\\
POSE~\cite{yang2023progressive} & 84.29	& 91.93	&& 78.69 & 87.20\\
DNA-Det~\cite{yang2022aaai} & 96.98	& 99.58	&& 84.35 & 92.36\\
Ours & 97.06 & 99.46 && 87.12 & 94.25\\
% Ours (training) & \\
\bottomrule[1pt]
\end{tabular}
\end{table}

% PRNU~\cite{marra2019gans}, Yu \etal~\cite{yu2019attributing}, DCT-CNN~\cite{frank2020leveraging}, DNA-Det~\cite{yang2022aaai}, and POSE~\cite{yang2023progressive}.

==> Tables/vary_sd_configs.tex <==
\begin{table}[htbp]
\centering
\caption{Robustness analysis on different diffusion generation configurations.}
\label{tab:vary_sd_configs}
\scalebox{1.1}{
\begin{tabular}{lccccccccc}
\toprule[1pt]
\multirow{2}{*}{Varied Configs} & \multicolumn{2}{c}{Verification} &&\multicolumn{2}{c}{Identification} \\  
\cmidrule{2-3} \cmidrule{5-6} 
& Acc & AUC && Acc & F1 \\
\midrule
None & \\
Sampler & \\
Sampling Step & \\ 
Resolution & \\
Guidance Scale & \\
\bottomrule[1pt]
\end{tabular}}
\end{table}



==> Tables/volume_compare.tex <==
\begin{table}[htbp]
\centering
\caption{Compare the relative percentages of volume against the total volume of all synthesized models when reducing each synthesis options.}
\label{tab:volume_compare}
\begin{tabular}{cccccccccc}
\toprule[1pt]
Models & All & w/o K & w/o L & w/o S  \\  
Relative Volume & 1 & 9.08E-09 & 1.05E-01 & 1.25E-01 \\
\midrule
Models & w/o U  & w/o A & w/o N & w/o seed \\  
Relative Volume & 7.02E-10 & 2.87E-02 & 3.67E-04 & 1.03E-03 \\
\bottomrule[1pt]
\end{tabular}
\end{table}

==> packages/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}
% for widebar
\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
%The bar will be moved to the right by a half of \macc@kerna, which is computed by amsmath:
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%If there's a superscript following the bar, then no negative kern may follow the bar;
%an additional {} makes sure that the superscript is high enough in this case:
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
%Use a separate algorithm for single symbols:
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
%Enable nesting of accents:
    \let\mathaccent\save@mathaccent
%If there's more than a single symbol, use the first character instead (see below):
    \if#32 \let\macc@nucleus\first@char \fi
%Determine the italic correction:
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
%Now \dimen@ is the italic correction of the symbol.
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
%Now \@tempdima is the width of the symbol.
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
%Now \dimen@ = (italic correction / 3) - (Breite / 10)
    \ifdim\dimen@>\z@ \dimen@0pt\fi
%The bar will be shortened in the case \dimen@<0 !
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
%Place the combined final kern (-\dimen@) if it is >0 or if a superscript follows:
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
%The following initialises \macc@kerna and calls \mathaccent:
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
%If the argument consists of more than one symbol, and if the first token is
%a letter, use that letter for the computations:
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{(\ref{#1})}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
% \def\reta{{\textnormal{$\eta$}}}
% \def\ra{{\textnormal{a}}}
% \def\rb{{\textnormal{b}}}
% \def\rc{{\textnormal{c}}}
% \def\rd{{\textnormal{d}}}
% \def\re{{\textnormal{e}}}
% \def\rf{{\textnormal{f}}}
% \def\rg{{\textnormal{g}}}
% \def\rh{{\textnormal{h}}}
% \def\ri{{\textnormal{i}}}
% \def\rj{{\textnormal{j}}}
% \def\rk{{\textnormal{k}}}
% \def\rl{{\textnormal{l}}}
% % rm is already a command, just don't name any random variables m
% \def\rn{{\textnormal{n}}}
% \def\ro{{\textnormal{o}}}
% \def\rp{{\textnormal{p}}}
% \def\rq{{\textnormal{q}}}
% \def\rr{{\textnormal{r}}}
% \def\rs{{\textnormal{s}}}
% \def\rt{{\textnormal{t}}}
% \def\ru{{\textnormal{u}}}
% \def\rv{{\textnormal{v}}}
% \def\rw{{\textnormal{w}}}
% \def\rx{{\textnormal{x}}}
% \def\ry{{\textnormal{y}}}
% \def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
% \newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\JS}{D_{\mathrm{JS}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\newcommand{\e}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\ea}{\begin{equation*}}
\newcommand{\eea}{\end{equation*}}

\newcommand{\rar}{\rightarrow}
\newcommand{\lar}{\leftarrow}
\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\lb}{\left\{}
\newcommand{\rb}{\right\}}
\newcommand{\ls}{\left[}
\newcommand{\rs}{\right]}

\newcommand{\bvec}[1]{\ensuremath{\begin{bmatrix}#1\end{bmatrix}}}
\newcommand{\pvec}[1]{\ensuremath{\begin{pmatrix}#1\end{pmatrix}}}

% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}

% \DeclareMathOperator{\sign}{sign}
% \DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

